Differentiable Solver Search for Fast Diffusion Sampling

Diffusion models have demonstrated remarkable generation quality but at the cost of numerous function evaluations. Recently, advanced ODE-based solvers have been developed to mitigate the substantial computational demands of reverse-diffusion solving under limited sampling steps. However, these solvers, heavily inspired by Adams-like multistep methods, rely solely on t-related Lagrange interpolation. We show that t-related Lagrange interpolation is suboptimal for diffusion model and reveal a compact search space comprised of time steps and solver coefficients. Building on our analysis, we propose a novel differentiable solver search algorithm to identify more optimal solver. Equipped with the searched solver, rectified-flow models, e.g., SiT-XL/2 and FlowDCN-XL/2, achieve FID scores of 2.40 and 2.35, respectively, on ImageNet256 with only 10 steps. Meanwhile, DDPM model, DiT-XL/2, reaches a FID score of 2.33 with only 10 steps. Notably, our searched solver outperforms traditional solvers by a significant margin. Moreover, our searched solver demonstrates generality across various model architectures, resolutions, and model sizes.

==> tables/compare_fmddpm.tex <==
\begin{minipage}{.49\textwidth}
\scalebox{0.5}{
    \begin{tabular}{lcccccc}
    \toprule
    \multicolumn{6}{l}{\bf{Class-Conditional ImageNet} 256$\times$256} \\
    \toprule
    Model & Steps & FID$\downarrow$   & sFID$\downarrow$  & IS$\uparrow$     & Precision$\uparrow$ & Recall$\uparrow$ \\
    \toprule
    {DiT-XL/2} & 250 & {3.04} & {5.02} & {240.82} & 0.84 & 0.54 \\
    \bottomrule
    \end{tabular}
}
\end{minipage}

==> tables/vis_coeffs.tex <==
\begin{figure}
    \captionsetup[subfigure]{labelformat=empty}
   \subfloat[Seached Solver Coefficients $c_i^j$ \label{fig:vis_coefficients}]{
        \includegraphics[width=0.65\linewidth]{NeuralSolver/figs/coeffs.png}
    } 
   \subfloat[Seached Normalized Timestep $t_i$ \label{fig:vis_timesteps}]{
        \includegraphics[width=0.35\linewidth]{NeuralSolver/figs/times.png}
    }
    \caption{\textbf{Visualization of Searched Solver Parameters.} {\small . }}
    \label{fig:vis_solver}
    \vspace{-2em}
\end{figure}
